ABot-AgentOS: A General Robotic Agent OS with Lifelong Multi-modal Memory

Recent VLM and VLA systems have improved robotic perception and action prediction, yet long-horizon embodied agents still require a general runtime layer for reasoning, memory, tool use, verification, and cross-embodiment execution. We present ABot-AgentOS, a general robotic Agent Operating System that sits above low-level controllers and provides a deliberative agent layer for scene-conditioned planning, context-isolated skill execution, multi-stage verification, multi-modal memory, and edge-cloud collaboration. To evaluate such systems, we introduce EmbodiedWorldBench, an executable benchmark with 16 indoor, outdoor, and hybrid scenes, four difficulty levels, and over 200 tasks involving navigation, object search, NPC dialogue, dynamic events, and trace-grounded scoring. ABot-AgentOS further introduces Universal Multi-modal Graph Memory, a persistent source-grounded substrate that converts dialogue, visual observations, spatial context, temporal relations, and task traces into typed nodes and edges. A failure-driven self-evolution loop converts diagnosed memory failures into gated runtime evo-assets that are promoted only to later evaluation splits, preventing current-split ground-truth leakage while enabling continual improvement. On an initial EmbodiedWorldBench subset, ABot-AgentOS improves over a single-controller baseline in both task success and goal completion. Across memory benchmarks, ABot-AgentOS Static achieves 87.5 on LoCoMo, 59.9 on OpenEQA EM-EQA, 88.6 on Mem-Gallery, and 76.5 Acc@All on NExT-QA; self-evolution further improves LoCoMo to 88.7, OpenEQA to 60.4, and Mem-Gallery to 89.0. These results suggest that a general Agent OS layer can improve long-horizon embodied execution while providing persistent, auditable memory for continual interaction.

==> sections/2_4_memory.tex <==
% ===========================================================================
% Edge-Cloud Collaborative Memory Management
% Usage: \input{section_memory_en} in your main document
% Required packages (ensure loaded in preamble):
%   \usepackage{booktabs, graphicx, amssymb, amsmath}
%   \usepackage{tikz}
%   \usetikzlibrary{arrows.meta, positioning}
% ===========================================================================

% \subsection{Edge-Cloud Collaborative Memory Management}
% \label{sec:memory-sync}

% \subsubsection{Problem Statement}

% During patrol, an on-device robot continuously acquires visual memories, each corresponding to a detected entity in the scene.
% These memories exhibit two inherent dimensions of heterogeneity:

% \begin{enumerate}
%     \item \textbf{Task relevance varies.} Traffic cones and construction barriers should trigger rerouting alerts for other devices; fire hydrants serve as localization landmarks. An undifferentiated memory store cannot support task-aware retrieval.
%     \item \textbf{Privacy sensitivity varies.} Faces and personal belongings are bound to specific individuals---disseminating them without sanitization violates privacy principles. In contrast, environmental information (road hazards, construction zones) is a public resource suitable for sharing.
% \end{enumerate}

% The core challenge is to automatically identify both dimensions at ingest time and enforce a ``never leak, rather under-share'' policy during cross-device synchronization.

% % ---------------------------------------------------------------------------
% \subsubsection{Method}
% \label{subsec:method}

% \paragraph{Two-Dimensional Classification}
% Rather than deferring relevance and privacy decisions to computationally expensive vision-language models, we adopt a prior-knowledge-driven approach: a compact set of task-specific priors defines which entities merit storage (task relevance) and, among stored records, which may be shared across devices (privacy sensitivity).
% This serves as a lightweight selective gating mechanism that eliminates model inference from the critical path while remaining extensible to model-assisted refinement.
% Each memory record is accordingly annotated with two orthogonal attributes (Table~\ref{tab:dimensions}), determined by deterministic rules and keyword matching.

% \begin{table}[ht]
% \centering
% \caption{Two-dimensional memory classification schema.}
% \label{tab:dimensions}
% \begin{tabular}{lll}
% \toprule
% Dimension & Values & Determination \\
% \midrule
% \texttt{sensitivity} & high / low & Whether bound to a specific individual \\
% \texttt{nav\_category} & hazard / poi / landmark / person / object & Task relevance \\
% \bottomrule
% \end{tabular}
% \end{table}

% A record is shareable if and only if its sensitivity is low; only shareable records are eligible for promotion to common memory.

% The open-vocabulary detector is configured with a task-specific keyword list that encodes task priors; only entities matching predefined categories (e.g., traffic cone $\mapsto$ hazard, fire hydrant $\mapsto$ landmark) are detected and enter the memory pipeline---front-gating irrelevant observations at perception time.
% Because the detector operates on natural-language prompts, novel entity types can be incorporated by extending the keyword list without retraining or rule modification, yielding a degree of generalization within the prior-based framework.

% The current instantiation applies three priority-ordered \textbf{sensitivity rules}.
% A record is classified as \textit{high} sensitivity if any of the following conditions holds; otherwise it defaults to \textit{low}:
% \begin{enumerate}
%     \item The entity has a \texttt{belongs\_to} relation referencing a person entity;
%     \item The entity category is \texttt{person}, or a face embedding is associated;
%     \item The description text contains a known person name or matches a privacy keyword.
% \end{enumerate}

% % ---------------------------------------------------------------------------
% \paragraph{Private--Common Memory Synchronization}
% The system separates memories into \textit{private memory} (edge-local, per-device) and \textit{common memory} (cloud-hosted, shared across devices).
% As shown in Figure~\ref{fig:sync-arch}, synchronization follows an offline-first protocol.

% \begin{figure}[t]
% \centering
% \begin{tikzpicture}[
%     node distance=0.8cm and 2.8cm,
%     box/.style={draw, rounded corners, minimum width=3.0cm, minimum height=2.0cm, align=center, font=\small},
%     arrow/.style={-{Stealth[length=3mm]}, thick},
%     lbl/.style={font=\footnotesize, align=center}
% ]
%     % Nodes
%     \node[box] (A) {Private Memory\\(Device A)\\[3pt]\footnotesize detect $\rightarrow$ classify\\[-2pt]\footnotesize $\rightarrow$ upload};
%     \node[box, right=of A] (cloud) {Common Memory\\(Cloud)\\[3pt]\footnotesize store \&\\[-2pt]\footnotesize deduplicate};
%     \node[box, right=of cloud] (B) {Private Memory\\(Device B)\\[3pt]\footnotesize download $\rightarrow$ dedup\\[-2pt]\footnotesize $\rightarrow$ merge};

%     % Arrows
%     \draw[arrow] (A) -- node[above, lbl] {upload\\(shareable only)} (cloud);
%     \draw[arrow] (cloud) -- node[above, lbl] {query \& fetch} (B);
% \end{tikzpicture}
% \caption{Overview of private--common memory synchronization. Only low-sensitivity records are promoted to common memory; downloaded records are marked non-re-shareable to prevent uncontrolled propagation.}
% \label{fig:sync-arch}
% \end{figure}

% Three design principles govern the architecture:
% \begin{itemize}
%     \item \textbf{Offline-first:} Private memory is the single source of truth; full functionality is preserved without network connectivity.
%     \item \textbf{Private by default:} Memories remain in private storage unless explicitly classified as low-sensitivity and promoted to common memory.
%     \item \textbf{No re-propagation:} Records downloaded from common memory are automatically marked as non-shareable.
% \end{itemize}

% % ---------------------------------------------------------------------------
% \paragraph{Receiver-Side Deduplication}
% The receiving device applies a two-strategy deduplication check (embedding cosine similarity and keyword Jaccard overlap, with configurable thresholds) on each incoming record to suppress redundant entries.
% Records surviving both checks are merged into private memory as non-shareable.

% % ---------------------------------------------------------------------------
% \subsubsection{Functional Verification}

% We verify the pipeline logic on two synthetic scenarios (4 frames each, generated via text-to-image synthesis) using an open-vocabulary detector for entity extraction.
% A total of 29 memory records are extracted across 7 entity categories.
% All records are classified consistently with the rule design: the 5 person-category records are correctly assigned high sensitivity and blocked from promotion to common memory, while all 24 environmental records receive low-sensitivity labels and pass the shareability gate.
% Dynamic vocabulary extension enables detection of user-specified categories beyond the default set (e.g., bench, thermos), confirming that the prior-based classification accommodates novel entity types without rule modification.

% % ---------------------------------------------------------------------------
% \subsubsection{Summary}

% This module implements automatic two-dimensional classification and privacy-safe cloud synchronization of visual memories.
% The classified memory store provides a standardized query interface (category-filtered, location-aware) designed to support downstream navigation and planning modules with task-specific retrieval without exposing raw sensor data.


\subsection{Edge--Cloud Collaborative Memory Management}
\label{sec:memory-sync}

Embodied agents continuously acquire heterogeneous memories during interaction with the physical world, including maps, semantic landmarks, obstacles, objects, and human-related observations. 
While public environmental memories, such as roadblocks, construction areas, and navigational landmarks, can improve multi-agent collaboration when shared, privacy-sensitive memories, such as faces, personal belongings, or person-associated objects, must remain local. 
To address this conflict, we design an edge--cloud collaborative memory system that separates private memory on the robot from common memory in the cloud.

\paragraph{Memory Partition.}
Each robot maintains a \emph{private memory} at the edge, which stores all locally perceived memories, including map memory, semantic memory, and multi-modal memory. 
The cloud maintains a \emph{common memory} that only contains public, low-sensitivity memories useful for collective navigation and task execution. 
This design follows a private-by-default principle: a memory item is never uploaded unless it is explicitly classified as shareable.

\paragraph{Privacy-aware Memory Gating.}
For each newly generated memory item, the system performs a privacy judgment before synchronization. 
A memory is regarded as non-shareable if it contains or is associated with personally identifiable information, including persons, faces, names, personal objects, or ownership relations to a specific individual. 
In contrast, public environmental information, such as maps, traffic cones, barriers, road damage, and static landmarks, is classified as shareable.


To evaluate the reliability of the privacy protection mechanism, we constructed a dedicated dataset for privacy classification and upload-decision testing. Experimental results show that the system achieves over 99\% accuracy in identifying whether a memory item is suitable for cloud synchronization. This high-accuracy privacy judgment significantly reduces the risk of uploading sensitive user or environment-specific information, while still allowing non-sensitive public knowledge to be shared across robots. As a result, the proposed memory system balances two key requirements of embodied intelligence: preserving user privacy through edge-side private memory, and enhancing group-level collaboration through cloud-side common memory.



==> sections/5router.tex <==
\section{Router}  
\label{sec:router}  

==> sections/intro-save.tex <==
\section{Introduction}
\label{sec:intro}

The ultimate goal of robotics should not be to develop specialized skills for specific hardware, but to build a general embodied agent~\cite{pi_0.5,shukor2025smolvla,eo1,zheng26}---similar to the human brain---that can operate across diverse robotic bodies, thereby realizing the vision of ``one mind, multiple forms''. Such an agent must perceive its environment, understand natural language instructions, reason about actions, and learn from interaction~\cite{rt2,liu2026rdt2,cheang2025gr,zheng25}. Despite decades of progress, this vision remains unrealized. Embodied intelligence has yet to reach its transformative moment.
% 机器人领域的最终目标不应是为特定硬件开发专用技能，而应是构建一种通用的具身智能体——类似于人类大脑——能够运行于各种机器人本体之上，从而实现“一脑多形”的愿景。这种智能体必须能感知环境、理解自然语言指令、推理行为并从交互中学习。尽管已有数十年的发展，这一愿景仍未实现，具身智能尚未迎来其突破性时刻。

We identify three key limitations. First, data scale has not reached a critical threshold. Unlike standard vision-language data, embodied data require precise action labels, which are expensive and slow to collect. Most current approaches rely on pre-training sets limited to a single robot type or platform. While effective for narrow deployment, this restricts the development of general policies by limiting exposure to diverse morphologies and task distributions. Second, data quality varies widely and lacks standardization. Action representations, coordinate systems, and control frequencies differ across datasets, making it difficult for models to extract common patterns across embodiments. The resulting fragmentation introduces noise and weakens learning, as models must allocate capacity to memorize idiosyncrasies rather than acquire transferable skills. Third, existing pre-training paradigms are mismatched. Most Vision-Language-Action (VLA) models start from Vision-Language Models (VLMs), whose visual encoders focus on semantic recognition rather than 3D structure or physical dynamics. Yet embodied behavior demands fine spatial understanding and causal reasoning---capabilities that cannot be acquired from 2D supervision alone, nor easily added through mechanisms such as Chain-of-Thought, because such methods operate at the reasoning level without enriching the underlying perceptual representation. Achieving general embodied intelligence therefore requires systematic improvements in data, representation, and training design.
% 我们指出了三个关键限制：第一，数据规模尚未达到临界点。与常规视觉-语言数据不同，具身数据需要精确的动作标注，采集成本高且耗时。现有方法大多依赖单一机器人或平台的数据集进行预训练。虽然适用于局部部署，但这种做法限制了对多样化形态和任务分布的接触，阻碍了通用策略的发展。第二，数据质量参差不齐且缺乏标准化。动作表示、坐标系和控制频率在不同数据集中各不相同，导致模型难以提取跨本体的共性知识。由此产生的碎片化引入了噪声，削弱了学习效果，因为模型不得不将容量用于记忆特异性模式，而非习得可迁移技能。第三，当前的预训练范式存在错配。大多数视觉-语言-动作（VLA）模型基于视觉-语言模型（VLM）初始化，其视觉编码器侧重语义识别，而非三维结构或物理动态建模。然而，具身行为需要精细的空间理解与因果推理能力，这些无法仅通过二维监督获得，也无法通过思维链等机制轻易弥补，因为此类方法作用于推理层面，并未增强底层感知表征。因此，实现通用具身智能需要在数据、表示和训练设计上进行系统性改进。

We address a practical question: given the high cost and hardware dependence of collecting robotic data, can we integrate global open-source datasets---currently isolated in silos---into a unified foundation for training hardware-agnostic VLA models? This suggests a new direction: instead of emerging from closed, proprietary systems, embodied intelligence can grow through the reorganization of public knowledge and incremental capability building, where shared infrastructure enables cumulative progress across research groups.
% 我们探讨一个实际问题：鉴于机器人数据采集的成本高昂且依赖硬件，能否将全球开源数据——目前分散在各个孤岛中——整合为统一基础，用于训练不依赖特定硬件的VLA模型？这指向一种新方向：具身智能不再源于封闭私有系统，而是通过公共知识的重构与能力的逐步积累而成长，其中共享基础设施支持研究团队间的持续进展。

To this end, we introduce \VLAFM{}, a unified approach that jointly optimizes data processing and model architecture. We combine six major open-source datasets---including OXE~\cite{o2024oxe}, OXE-AugE~\cite{ji2025oxeauge}, Agibot-Beta~\cite{agibotbeta}, RoboCoin~\cite{wu2025robocoin}, RoboMind~\cite{wu2024robomind}, and Galaxea~\cite{jiang2025galaxea} --- to form a mixed training set of over 6 million trajectories, the largest such collection outside proprietary efforts. To resolve inconsistencies in action format, coordinate system, and sampling rate, we define a standardized preprocessing pipeline. All actions are converted to delta actions in the end-effector frame; rotations are encoded using rotation vectors to avoid singularities; and we apply a pad-to-dual strategy to support both single-arm and dual-arm tasks within a shared framework. This unified data foundation breaks down barriers between datasets and enables robust cross-embodiment generalization by aligning both geometric and temporal structures across sources.
% 为此，我们提出\VLAFM{}，一种协同优化数据处理与模型架构的统一方法。我们整合六个主要开源数据集——包括OXE、OXE-AugE、Agibot-Beta和RoboCoin——构建了超过600万条轨迹的混合训练集，是目前非私有体系中规模最大的集合。为解决动作格式、坐标系和采样率的不一致，我们定义了标准化预处理流程：所有动作转换为末端执行器坐标系下的增量动作；旋转使用旋转向量编码以避免奇异性；采用pad-to-dual策略，在共享框架下支持单臂与双臂任务。这一统一的数据基础打破了数据壁垒，通过在源间对齐几何与时间结构，实现了强大的跨本体泛化能力。

On the modeling side, we build on the ``VLM + Action Expert'' architecture and introduce two core innovations. First, most VLA models~\cite{GR00T,team2024octo,li2024cogact,reuss2025flower} train the policy to predict noise---either $\epsilon$-prediction or $v$-prediction---which is unstructured, meaningless, and often includes invalid actions such as jittering or discontinuities. These noisy targets spread across high-dimensional space, requiring large model capacity and leading to inefficient learning. Inspired by JiT~\cite{JIT} compilation, we propose the \textit{``Action Manifold Hypothesis''}: successful actions do not scatter randomly but lie on a low-dimensional, smooth manifold shaped by physics, task goals, and environmental constraints. Based on this, we design the Action Manifold Learning (AML) mechanism, where the DiT backbone directly predicts clean action sequences. This shifts the learning objective from fitting noise to projecting onto feasible action manifolds, improving decoding speed and policy stability by reducing output uncertainty. Second, to improve spatial understanding, we add modular components that either inject scene-level structural priors via VGGT~\cite{wang2025vggt} or fuse multi-view observations generated by Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport}, allowing flexible enhancement without modifying the main architecture. These modules act as plug-and-play experts that enrich perception with geometry-aware features, addressing the representational gap left by standard VLMs.
% 在模型方面，我们在“VLM + 动作专家”架构基础上提出两项核心创新。首先，多数VLA模型训练策略预测噪声（如ε预测或v预测），这些噪声无结构、无意义，常包含抖动或不连续等无效动作，散布于高维空间，要求模型具备大容量，导致学习效率低下。受JiT启发，我们提出“动作流形假说”：成功动作并非随机分布，而受限于物理规律、任务目标和环境约束，聚集在低维平滑流形上。基于此，我们设计AML机制，使DiT主干直接预测干净的动作序列，将学习目标从拟合噪声转变为向可行流形投影，通过减少输出不确定性，显著提升解码速度与策略稳定性。其次，为增强空间理解，我们引入模块化组件，通过VGGT注入场景级结构先验，或融合LongCat生成的多视角观测特征，可在不修改主干的情况下灵活增强能力。这些模块作为即插即用的专家，通过几何感知特征丰富感知能力，弥补了标准VLM留下的表征差距。

We perform full ablation studies under a consistent training setup, showing that data standardization, architectural changes, and training redesign are orthogonal and their benefits accumulate. Our model achieves average success rates of 98.6\%, 80.5\% and 58.3\% on benchmarks including LIBERO~\cite{liu2023libero}, LIBERO-Plus~\cite{fei25libero-plus}, and RoboCasa GR1 Tabletop Tasks~\cite{GR00T}, outperforming strong baselines such as $\pi_{0.5}$~\cite{pi_0.5}, UniVLA~\cite{bu2025univla}, and openVLA-OFT~\cite{kim2024openvla}. These results confirm a complete pathway---from data to architecture to capability---that enables high-performance, generalizable embodied intelligence through systematic engineering, even without private data. Notably, the gains from each component remain consistent across platforms, suggesting that the learned representations generalize beyond dataset-specific artifacts. We will fully release our data processing and training code to support community-driven progress toward open, shared, and evolving general-purpose robotics.
% 我们在统一训练框架下进行了完整消融实验，结果表明数据标准化、架构改进与训练设计三者相互正交且收益可叠加。模型在Libero、Libero-Plus、和RoboCasa等多个基准上分别取得98.6%、80.5%、58.3%的平均成功率，显著优于pi0、uniVLA和openVLA-OFT等先进方法。结果验证了一条从数据到架构再到能力的完整技术路径，证明即使没有私有数据，也能通过系统工程构建高性能、强泛化的具身智能。值得注意的是，各组件带来的增益在不同平台上保持一致，表明所学表征超越了数据集特异性偏差。我们将全面开源数据处理与训练代码，推动社区共建共享、持续进化的通用机器人生态发展。



==> sections/intro_new.tex <==
\section{Introduction}
\label{sec:intro}

\section{Introduction}

The ultimate goal of robotics is to build general embodied agents that operate across diverse robotic bodies, realizing the vision of ``one brain, many forms''~\cite{rt2,liu2026rdt2,cheang2025gr}. While Large Language Models (LLMs) have achieved universality in the digital realm, embodied intelligence remains fragmented—policies trained on one robot rarely transfer to another, and high-level semantic reasoning struggles to translate into low-level physical precision. We ask a critical question: \textit{Why has the ``ChatGPT Moment'' for robotics not yet arrived?}
% 机器人学的终极目标是构建能够跨多种机器人本体运行的通用具身智能体，实现“一脑多形”（one brain, many forms）的愿景~\cite{rt2,liu2026rdt2,cheang2025gr}。尽管大语言模型（LLMs）已在数字领域实现普适性，具身智能却仍处于碎片化状态——针对单一机器人训练的策略难以迁移到其他平台，高层语义推理也难以转化为底层物理操作的精确控制。我们提出一个关键问题：为何机器人领域尚未迎来属于自己的“ChatGPT 时刻”？

We argue that the field is currently blocked by two invisible walls: the \textit{Curse of Data Heterogeneity} and the \textit{Manifold Misalignment}. Unlike the standardized text data that fueled the LLM revolution, robotic data is trapped in silos. High costs and diverse hardware create a ``Tower of Babel'', where the open-source community possesses vast but fragmented data, while proprietary models build moats around standardized but closed ecosystems. Furthermore, existing Vision-Language-Action (VLA) models often treat actions as unstructured noise (e.g., diffusion noise prediction~\cite{GR00T}), ignoring the physical reality that valid motions follow strict kinematic laws rather than random distributions.
% 我们认为，当前领域被两堵“隐形高墙”所阻隔：数据异构性诅咒（Curse of Data Heterogeneity）与流形错位（Manifold Misalignment）。与推动LLM革命的标准化文本数据不同，机器人数据深陷孤岛困境。高昂成本与硬件多样性构筑起一座“巴别塔”：开源社区虽拥有海量数据，却高度碎片化；而私有模型则围绕标准化但封闭的生态系统筑起护城河。此外，现有视觉-语言-动作（VLA）模型常将动作视为无结构的噪声（如基于扩散的噪声预测~\cite{GR00T}），忽视了物理现实——有效运动遵循严格的运动学规律，而非随机分布。

To shatter these barriers and democratize generalist robotics, we introduce \VLAFM{}, a unified foundation model built on the philosophy of ``United We Scale.'' Our primary contribution is not merely a model, but a reproducible \textbf{Open-Source Data Curation Pipeline} designed to break the data monopoly. We demonstrate that the community does not need to wait for a single massive dataset release; we already possess the critical mass—if properly refined. We systematically integrate six major disparate open-source datasets—including OXE~\cite{o2024oxe}, OXE-AugE~\cite{ji2025oxeauge}, Agibot-Beta~\cite{agibotbeta}, and RoboCoin~\cite{wu2025robocoin}—into a coherent training set of over \textbf{6 million trajectories}, the largest non-proprietary collection to date. Crucially, we establish a rigorous standardization protocol: unifying action spaces into delta-end-effector poses, encoding rotations via rotation vectors to avoid singularities, and applying a pad-to-dual strategy to support heterogeneous morphologies. This pipeline transforms scattered ``data fragments'' into high-octane fuel, proving that with rigorous curation, community-aggregated data can rival proprietary data moats.
% 为打破这些壁垒、推动通用机器人技术的民主化，我们提出 \VLAFM{}，一个基于“聚力方能规模化”（United We Scale）理念构建的统一基础模型。我们的核心贡献不仅是一个模型，更是一套可复现的开源数据整理管道，旨在瓦解数据垄断。我们证明：社区无需等待单一超大规模数据集的发布——我们已具备关键数据体量，只需加以精炼。我们系统性整合六大异构开源数据集（包括 OXE~\cite{o2024oxe}、OXE-AugE~\cite{ji2025oxeauge}、Agibot-Beta~\cite{agibotbeta} 与 RoboCoin~\cite{wu2025robocoin}），构建出包含逾600万条轨迹的统一训练集，成为迄今规模最大的非私有数据集合。尤为关键的是，我们建立了一套严格标准化协议：将动作空间统一为末端执行器位姿增量（delta-end-effector poses），采用旋转矢量（rotation vectors）编码旋转以避免奇异性，并引入“填充至双臂”（pad-to-dual）策略以支持异构形态。该管道将零散的“数据碎片”转化为高能燃料，证明经严谨整理的社区聚合数据足以媲美私有数据护城河。

Building on this unified foundation, we propose the \textbf{Action Manifold Hypothesis} to resolve the modeling misalignment. We posit that successful robotic actions do not scatter randomly in high-dimensional space but reside on a low-dimensional, smooth manifold shaped by physics and task constraints. Instead of the prevailing practice of fitting unstructured noise, we introduce \textbf{Action Manifold Learning (AML)}. This mechanism guides our DiT-based policy to project visual intent directly onto this feasible action manifold, filtering out physical jitter and significantly accelerating inference by reducing output uncertainty. To further bridge the gap between 2D semantics and 3D execution, we incorporate plug-and-play spatial experts, such as VGGT~\cite{wang2025vggt} and Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport}, which inject scene-level structural priors without altering the core architecture.
% 基于这一统一基础，我们提出动作流形假设（Action Manifold Hypothesis）以解决建模错位问题。我们主张：成功的机器人动作并非在高维空间中随机散布，而是栖居于一个由物理规律与任务约束塑造的低维、平滑流形之上。我们摒弃拟合无结构噪声的主流做法，引入动作流形学习（Action Manifold Learning, AML）。该机制引导基于扩散Transformer（DiT）的策略将视觉意图直接投影至可行动作流形，滤除物理抖动，并通过降低输出不确定性显著加速推理。为弥合2D语义与3D执行间的鸿沟，我们进一步集成即插即用的空间专家模块（如 VGGT~\cite{wang2025vggt} 与 Qwen-Image-Edit~\cite{wu2025qwenimagetechnicalreport}），在不改动核心架构的前提下注入场景级结构先验。

Our results confirm that scale and structure must go hand in hand. Under a consistent training setup, \VLAFM{} achieves state-of-the-art performance, recording average success rates of \textbf{98.6\%} on LIBERO~\cite{liu2023libero}, 80.5\% on LIBERO-Plus~\cite{fei25libero-plus}, and 58.3\% on RoboCasa GR1 tasks~\cite{GR00T}, significantly outperforming strong baselines like $\pi_{0.5}$~\cite{pi_0.5} and OpenVLA~\cite{kim2024openvla}. These gains remain consistent across platforms, suggesting that our standardized representations generalize beyond dataset-specific artifacts. We will fully release our data curation pipeline and training code, providing a blueprint for the community to collaboratively build a shared, evolving, and truly open general-purpose robotic brain.
% 实验结果证实：规模与结构必须协同演进。\VLAFM{} 在统一训练设置下取得当前最优性能，在 LIBERO~\cite{liu2023libero}、LIBERO-Plus~\cite{fei25libero-plus} 与 RoboCasa GR1 任务~\cite{GR00T} 上分别达到 98.6%、80.5% 与 58.3% 的平均成功率，显著超越 
 % ~\cite{pi_0.5} 与 OpenVLA~\cite{kim2024openvla} 等强基线模型。性能增益在不同平台间保持一致，表明我们的标准化表征可泛化至数据集特有伪影之外。我们将完整开源数据整理管道与训练代码，为社区协作构建一个共享、演进且真正开放的通用机器人“大脑”提供蓝图。



==> sections/subsec_4_4_rl_gigpo_llm_as_judge_standalone.tex <==
% Standalone Section 4.4 draft.
% Usage: copy this file into the target LaTeX project and include it with \input{...}.
% Required citation keys:
%   - zhou2024archer
%   - wei2025webagentr1
%   - wang2025ragen
%   - feng2025gigpo

\subsection{RL: Online Exploration with LLM-as-Judge Reward}
\label{sec:rl}

SFT gives the small policy a warm start from expert demonstrations. We then use online RL to improve recovery from its own mistakes through interaction. This follows recent multi-turn agent RL systems that move beyond static imitation~\citep{zhou2024archer,wei2025webagentr1,wang2025ragen}. This stage is challenging because embodied trajectories contain many tool calls, observations, and NPC responses. A terminal success signal is therefore too sparse for reliable credit assignment~\citep{wang2025ragen}. We use a frozen LLM-as-Judge reward provider to convert each rollout into turn-level and episode-level reward signals. During RL, the simulator remains fixed and only the small policy is updated.

\subsubsection{Training Architecture}

We build on the ROLL (Reinforcement Learning with Online Learning) framework:

\begin{itemize}
    \item \textbf{Policy (Actor):} the small LLM being trained. It is served by vLLM for efficient online generation and produces reasoning traces and structured tool calls.
    \item \textbf{Environment:} \texttt{DogSimulatedEnv}, an online RL wrapper around the GM/NPC-driven simulator introduced in the benchmark and SFT stages. It receives the policy's action, updates the simulated world state, and returns observations or execution feedback.
    \item \textbf{Reward Provider:} a frozen LLM-as-Judge evaluator. It reads the trajectory context, the current action, and the environment feedback, then produces turn-level and episode-level reward signals.
\end{itemize}

A critical design principle is role separation. The policy model is not the simulator model. The policy is the trainable small LLM, while the simulator is driven by a frozen large model. The LLM-as-Judge is also separated from policy optimization. It supplies reward signals but does not receive gradient updates during RL. This separation keeps the environment dynamics and reward landscape stable while the policy improves. The reward provider is fixed within each RL run; prompt self-evolution is performed outside the policy update loop and produces the next audited reward-provider snapshot.

The rollout sequence is an interleaved agent-environment trace. Policy-generated tokens and tool calls are optimized. In contrast, environment feedback, simulator messages, and LLM-as-Judge outputs are treated as context and masked out from the policy loss. This prevents the policy from being trained to imitate observations or reward explanations. The update therefore focuses on the model's own decisions.

\subsubsection{Reward Design}

The LLM-as-Judge provides two complementary reward signals for RL. The turn-level signal gives dense local feedback, while the episode-level signal evaluates global task completion. Section~\ref{sec:judge} introduces the self-evolving multi-tier reward engine that generates, audits, and refines these reward signals. Here, we focus on how the fixed reward outputs are consumed by policy optimization.

\paragraph{Turn-level reward.}
After each action, the frozen LLM-as-Judge assigns a turn-level reward:
\begin{equation}
r_{i,t}^{\mathrm{turn}}
=
J_{\mathrm{turn}}(s_{i,t},a_{i,t},o_{i,t+1}),
\end{equation}
Here, $s_{i,t}$ is the current decision context, and $a_{i,t}$ is the policy action. The term $o_{i,t+1}$ denotes the resulting observation or execution feedback. This reward evaluates whether the action fits the current embodied context, tool constraints, physical preconditions, task goal, and output-format requirements. Invalid tool names, malformed arguments, schema violations, and incomplete tool calls are incorporated as format penalties:
\begin{equation}
\hat r_{i,t}
=
r_{i,t}^{\mathrm{turn}}
+
r_{i,t}^{\mathrm{format}}.
\end{equation}
This signal provides dense local feedback: it tells the policy which intermediate actions are useful, redundant, unsafe, malformed, or inconsistent with the current context.

\paragraph{Episode-level reward and aggregation.}
After the trajectory terminates, the LLM-as-Judge assigns an episode-level reward:
\begin{equation}
r_i^{\mathrm{episode}}
=
J_{\mathrm{episode}}(\tau_i),
\end{equation}
which evaluates global task completion, efficiency, consistency, and completeness. This signal discourages locally plausible actions that fail to complete the overall task. We use the existing \texttt{step\_plus\_episode\_sum} merge strategy to form the trajectory return:
\begin{equation}
R_i
=
\sum_{t=1}^{T_i}\hat r_{i,t}
+
r_i^{\mathrm{episode}}.
\end{equation}
Thus, the return used by GiGPO contains both accumulated effective turn-level rewards and the terminal episode-level reward. Turn-level rewards address local credit assignment. Episode-level rewards preserve the long-horizon objective: the policy must still complete the task efficiently and coherently.

\subsubsection{Training Algorithm}

We adopt GiGPO (Group-in-Group Policy Optimization) for policy updates, with distributed rollout collection via Ray~\citep{feng2025gigpo}. GiGPO is well aligned with our robot-dog RL setting. Each training scenario defines a complete runnable world. Different rollouts from the same scenario can still diverge at both the trajectory level and the local decision level. We therefore use GiGPO in two complementary comparisons:
\begin{enumerate}
    \item \textbf{Trajectory-group comparison:} compares which rollout solves the same scenario better.
    \item \textbf{Anchor-state action comparison:} compares decisions made under comparable local states.
\end{enumerate}

\paragraph{Trajectory-group comparison.}
For each scenario, we initialize a group of parallel environments from the same initial state and sample multiple trajectories:
\begin{equation}
\mathcal{G}^{E}
=
\{\tau_1,\tau_2,\ldots,\tau_G\},
\quad
\tau_i
=
\{(s_{i,t},a_{i,t},o_{i,t+1})\}_{t=1}^{T_i}.
\end{equation}

Each scenario contains the task instruction, initial dog position, scene map, NPC configuration, obstacle layout, dynamic events, success criteria, and step budget. After each trajectory receives its merged return $R_i$, we compare trajectories within the same scenario:
\begin{equation}
A_i^{E}
=
\frac{
R_i-\mathrm{mean}(\{R_j\}_{j=1}^{G})
}{
\mathrm{std}(\{R_j\}_{j=1}^{G})+\epsilon
}.
\end{equation}
This trajectory-group advantage answers which complete trajectory is better under the same task and initial condition. In robot-dog tasks, local plausibility does not guarantee global success. Two rollouts may both move toward plausible regions. However, only one may ask the necessary NPC, trigger the correct door event, reject misleading clues, and report the correct destination within the step budget. The trajectory-group advantage therefore handles global credit assignment over the full embodied execution path.

\paragraph{Anchor-state action comparison.}
Beyond complete trajectories, robot-dog tasks also create repeated local decision contexts across rollouts. The policy may arrive at the same door, face the same blocked passage, or approach the same NPC. It may also observe the same candidate target or stand near the same destination region. When multiple trajectories reach the same or similar decision context, their actions form a step-level anchor-state group:
\begin{equation}
\mathcal{G}^{S}(c)
=
\{(j,u)\mid c_{j,u}\sim c\}.
\end{equation}
Here $c_{i,t}$ can include the current task goal, location or scene state, latest observation, and available tools. It can also include previous key actions, unresolved obstacles, and relevant social context. The social context may include the nearby NPC and its prior responses. This anchor-state group allows GiGPO to compare competing actions in similar embodied situations. Examples include asking an NPC for clarification versus leaving, speaking a door keyword versus rerouting, and verifying a candidate target versus prematurely reporting. For each action in such a group, we compute an anchor-state advantage from the effective turn-level reward:
\begin{equation}
A_{i,t}^{S}
=
\frac{
\hat r_{i,t}
-
\mathrm{mean}(\{\hat r_{j,u}:(j,u)\in \mathcal{G}^{S}(c_{i,t})\})
}{
\mathrm{std}(\{\hat r_{j,u}:(j,u)\in \mathcal{G}^{S}(c_{i,t})\})+\epsilon
}.
\end{equation}

\paragraph{Combined advantage.}
The final GiGPO advantage combines the trajectory-group advantage and the anchor-state advantage:
\begin{equation}
A_{i,t}^{\mathrm{GiGPO}}
=
A_i^{E}
+
\alpha A_{i,t}^{S}.
\end{equation}
If no comparable anchor-state group exists for a turn, we set $A_{i,t}^{S}=0$, so the update falls back to the trajectory-group advantage:
\begin{equation}
A_{i,t}^{\mathrm{GiGPO}}
=
A_i^{E}.
\end{equation}
This fallback is important because some embodied states are unique within a rollout group, such as one-off dynamic events or rare observation histories. In those cases, GiGPO avoids fabricating a local comparison and relies only on the trajectory-group advantage.

Overall, GiGPO converts LLM-as-Judge rewards into hierarchical relative advantages instead of using raw reward scores directly. The trajectory-group advantage handles global credit assignment over complete embodied trajectories. The anchor-state advantage handles local credit assignment over comparable robot-dog states. The resulting policy loss updates only the small policy model. Simulator outputs, environment feedback, and LLM-as-Judge outputs remain fixed and masked. Section~\ref{sec:judge} further describes this reward engine outside the RL update loop: LLM-as-Judge reward generation, Meta-Judge audit, and multi-agent self-evolution of the reward prompt.


==> sections/subsec_4_5_judge_model_draft.tex <==
This section introduces a self-evolving multi-tier reward engine for embodied agent evaluation and optimization. As shown in Figure, the engine converts embodied trajectories into dense reward signals, audits the reliability of those signals, and uses audit feedback to improve the reward prompt itself. The overall design is organized around three coupled components:
\begin{itemize}
    \item \textbf{LLM-as-Judge reward generation:} produces turn-level and episode-level reward signals from embodied trajectories.
    \item \textbf{Meta-Judge reasoning-level audit:} checks whether the judge's score and reasoning trace are reliable.
    \item \textbf{Multi-agent self-evolution:} converts low-quality judge cases into localized prompt updates with validation and rollback.
\end{itemize}

% \begin{figure}[!t]
% \centering
% \includegraphics[width=\linewidth]{figure/judge_system_overview_v9_cropped.pdf}
% \vspace{-0.4em}
% \caption{Overview of the self-evolving multi-tier reward engine. The system forms a closed loop that turns embodied trajectories into dense reward signals, audits the reliability of those rewards, and uses the audit results to improve the reward prompt. Module 1, LLM-as-Judge reward generation, decomposes each trajectory into turn-level rewards, episode-level rewards, and a final aggregated reward. Module 2, Meta-Judge audit, evaluates whether the judge's score and reasoning trace are supported by trajectory evidence and rubric constraints. Module 3, multi-agent self-evolution, clusters low-quality judge cases, analyzes prompt defects, refines local rubric components, and validates each update before acceptance or rollback.}
% \label{fig:judge_overview_v9}
% \end{figure}

\subsubsection{Multi-Tier Reward Signals with LLM-as-Judge}
\label{subsec:multi_tier_reward}

The first component in Figure generates reward signals from embodied trajectories. Instead of assigning only one outcome-level score, the judge decomposes evaluation into turn-level and episode-level rewards. The episode-level component is the global reward consumed by GiGPO in Section~\ref{sec:rl}. This decomposition is important for long-horizon embodied tasks, where a final success or failure signal is too sparse to explain which intermediate action caused the outcome~\citep{wei2025reinforcing}. In our design, the two levels play complementary roles:
\begin{itemize}
    \item \textbf{Turn-level reward:} provides dense supervision and finer credit assignment for individual actions.
    \item \textbf{Episode-level reward:} captures global execution quality that cannot be judged reliably from isolated turns alone.
\end{itemize}

At the turn level, the reward engine uses skill-aware routing to select the appropriate rubric for each action. This is necessary because embodied agents call heterogeneous skills, such as navigation, manipulation, visual question answering, and tool use, whose correctness criteria differ substantially. The turn-level judge therefore combines three mechanisms:
\begin{itemize}
    \item \textbf{Skill-aware routing:} routes each action to a skill-specific rubric instead of relying on a single generic rubric.
    \item \textbf{Hybrid scoring:} combines semantic LLM judgment with verifiable checks, including invalid tools, illegal commands, and missing temporal preconditions.
    \item \textbf{Action omission penalty:} detects actions that appear plausible locally but skip necessary causal steps.
\end{itemize}

At the episode level, the judge adds compact global signals for efficiency, consistency, and completeness~\citep{han2026swetrace}. These signals complement local turn rewards by discouraging trajectories that eventually succeed through inefficient, incoherent, or incomplete behavior:
\begin{itemize}
    \item \textbf{Efficiency:} penalizes redundant or repetitive execution.
    \item \textbf{Consistency:} checks whether the agent remains aligned with the original task.
    \item \textbf{Completeness:} measures whether required steps have been covered.
\end{itemize}

Given an embodied trajectory $\tau$ with $T$ evaluated action turns, the final reward is composed as:
\begin{equation}
R(\tau)=
\sum_{t=1}^{T}\hat{r}_{t}
+ \lambda_{\mathrm{eff}} R_{\mathrm{eff}}(\tau)
+ \lambda_{\mathrm{cons}} R_{\mathrm{cons}}(\tau)
+ \lambda_{\mathrm{comp}} R_{\mathrm{comp}}(\tau),
\label{eq:multi_tier_reward}
\end{equation}
where $\hat{r}_{t}$ is the effective turn-level reward after skill-aware routing, rule-based checks, LLM judgment, and omission penalties. $R_{\mathrm{eff}}$, $R_{\mathrm{cons}}$, and $R_{\mathrm{comp}}$ denote episode-level efficiency, consistency, and completeness rewards computed over the full trajectory. This formulation turns LLM-as-Judge from a static evaluator into a structured reward generator for embodied agent optimization~\citep{zheng2023judging}.

\subsubsection{Meta-Judge for Reasoning-Level Reward Audit}
\label{subsec:meta_judge_audit}

The second component in Figure audits the reliability of the reward signal. In practice, LLM-as-Judge outputs can contain scoring mistakes, missed evidence, rubric misapplication, or plausible but unsupported rationales~\citep{silva2026metajudging}. This risk is amplified in embodied settings, where the judge must reason over physical preconditions, tool constraints, temporal order, and task-specific preferences.

To address this issue, Meta-Judge does not directly judge whether the embodied agent acted correctly. Instead, it receives the first-order judge output, the highlighted turn, and the full trajectory context as audit evidence, and then asks whether the judge's score and reasoning are reliable under the relevant scoring rubric. For each audited turn, Meta-Judge scores judgment quality along five dimensions:
\begin{itemize}
    \item \textbf{Accuracy:} whether the assigned reward score is consistent with the skill-specific scoring rubric and supported by the audited trajectory evidence.
    \item \textbf{Logical soundness:} whether the reasoning forms a valid chain from trajectory evidence, through rubric application, to the final reward decision, without unsupported jumps or contradictions.
    \item \textbf{Completeness:} whether the judge covers the key embodied checks required for the audited turn, including tool choice, arguments, temporal preconditions, physical constraints, capability boundaries, and omitted or redundant actions.
    \item \textbf{Clarity:} whether the explanation states the evidence, applied rule, and score rationale in a structured and unambiguous way.
    \item \textbf{Feedback value:} whether the reasoning exposes sufficiently localized evidence and rule usage for downstream Meta-Judge filtering and prompt refinement, rather than providing only a generic score justification.
\end{itemize}

This reasoning-level audit is motivated by recent findings that LLM-as-Judge and generative reward models often expose judgment failures through their rationales: the reasoning trace can reveal unsupported evidence use, inconsistent rubric application, or other forms of rationale inconsistency~\citep{wang2026outcome}. Since human annotation for embodied trajectories is expensive, we use this rationale as a practical audit entry point: Meta-Judge checks whether the judge's explanation faithfully supports its reward decision before the output is trusted as a high-quality reward signal. These dimensions are aggregated into an overall quality score:
\begin{equation}
Q(x_t)=\sum_{k=1}^{5} w_k q_k,
\label{eq:meta_quality}
\end{equation}
where $x_t$ denotes the audited judge output, $q_k$ is the score of the $k$-th audit dimension, and $w_k$ is its weight. A sample is marked as a low-quality judge case when:
\begin{equation}
\mathrm{LowQualityJudgeCase}(x_t)=\mathbb{I}[Q(x_t)<\theta].
\label{eq:low_quality_case}
\end{equation}

These low-quality judge cases preserve diagnostic feedback rather than only binary error labels. They identify where the reward prompt is underspecified, ambiguous, or misaligned with embodied execution constraints, and provide the optimization signal for the next stage~\citep{li2025multiagent}.

\subsubsection{Multi-Agent Self-Evolution from Judge Audit Signals}
\label{subsec:structured_reward_optimization}

The third component in Figure converts low-quality judge cases into localized prompt updates. The goal is to improve the reward engine itself rather than treating judge errors as fixed noise. Generic prompt optimization methods usually optimize a monolithic prompt with task-level feedback~\citep{yang2024opro,khattab2023dspy}. In our setting, however, the reward prompt contains skill-specific rubrics, temporal precondition rules, reasoning examples, and output constraints. A global rewrite can repair one failure while damaging another stable skill. We therefore treat the reward prompt as editable structured components, following the broader idea of modular textual parameters and localized textual modification from execution feedback~\citep{he2026learning}.

The optimization loop is implemented as a multi-agent workflow. Each module handles one stage of the update process:
\begin{itemize}
    \item \textbf{Cluster:} groups low-quality judge cases by skill and failure type.
    \item \textbf{Analyzer:} identifies the defective rubric component and produces a structured revision plan.
    \item \textbf{Refiner:} applies localized edits to the relevant rubric or examples.
    \item \textbf{Validator:} re-evaluates the revised prompt on the full validation set and accepts the update only when it improves overall quality.
\end{itemize}

If a candidate update hurts full-set performance, per-skill behavior, or Meta-Judge quality, the system rolls back to the previous prompt snapshot. This makes prompt self-evolution auditable and controlled: the structured revision plan records what should be changed and why, while validation prevents overfitting to isolated bad cases.

Under the current validation setting, the initial Judge Model achieves roughly 60\% human alignment, while the Meta-Judge-driven self-evolution process improves alignment to above 90\%. This gain reflects the coupled effect of the full loop: LLM-as-Judge produces decomposed rewards, Meta-Judge turns unreliable judgments into diagnostic cases, and the multi-agent optimizer converts these cases into validated prompt updates.

Overall, the proposed reward engine closes the loop around reward production. It not only generates dense multi-tier rewards for embodied trajectories, but also audits and improves the judging process that produces those rewards. This allows the evaluation system to remain reliable as embodied skills, task distributions, and agent behaviors evolve.


==> subsec_4_5_judge_model_draft.tex <==
This section introduces a self-evolving multi-tier reward engine for embodied agent evaluation and optimization. As shown in Figure~\ref{fig:judge_overview_v9}, the engine converts embodied trajectories into dense reward signals, audits the reliability of those signals, and uses audit feedback to improve the reward prompt itself. The overall design is organized around three coupled components:
\begin{itemize}
    \item \textbf{LLM-as-Judge reward generation:} produces turn-level and episode-level reward signals from embodied trajectories.
    \item \textbf{Meta-Judge reasoning-level audit:} checks whether the judge's score and reasoning trace are reliable.
    \item \textbf{Multi-agent self-evolution:} converts low-quality judge cases into localized prompt updates with validation and rollback.
\end{itemize}

\begin{figure}[!t]
\centering
\includegraphics[width=\linewidth]{figure/judge_system_overview_v9_cropped.pdf}
\vspace{-0.4em}
\caption{Overview of the self-evolving multi-tier reward engine. The system forms a closed loop that turns embodied trajectories into dense reward signals, audits the reliability of those rewards, and uses the audit results to improve the reward prompt. Module 1, LLM-as-Judge reward generation, decomposes each trajectory into turn-level rewards, episode-level rewards, and a final aggregated reward. Module 2, Meta-Judge audit, evaluates whether the judge's score and reasoning trace are supported by trajectory evidence and rubric constraints. Module 3, multi-agent self-evolution, clusters low-quality judge cases, analyzes prompt defects, refines local rubric components, and validates each update before acceptance or rollback.}
\label{fig:judge_overview_v9}
\end{figure}

\subsubsection{Multi-Tier Reward Signals with LLM-as-Judge}
\label{subsec:multi_tier_reward}

The first component in Figure~\ref{fig:judge_overview_v9} generates reward signals from embodied trajectories. Instead of assigning only one outcome-level score, the judge decomposes evaluation into turn-level and episode-level rewards. The episode-level component is the global reward consumed by GiGPO in Section~\ref{sec:rl}. This decomposition is important for long-horizon embodied tasks, where a final success or failure signal is too sparse to explain which intermediate action caused the outcome~\citep{wei2025reinforcing}. In our design, the two levels play complementary roles:
\begin{itemize}
    \item \textbf{Turn-level reward:} provides dense supervision and finer credit assignment for individual actions.
    \item \textbf{Episode-level reward:} captures global execution quality that cannot be judged reliably from isolated turns alone.
\end{itemize}

At the turn level, the reward engine uses skill-aware routing to select the appropriate rubric for each action. This is necessary because embodied agents call heterogeneous skills, such as navigation, manipulation, visual question answering, and tool use, whose correctness criteria differ substantially. The turn-level judge therefore combines three mechanisms:
\begin{itemize}
    \item \textbf{Skill-aware routing:} routes each action to a skill-specific rubric instead of relying on a single generic rubric.
    \item \textbf{Hybrid scoring:} combines semantic LLM judgment with verifiable checks, including invalid tools, illegal commands, and missing temporal preconditions.
    \item \textbf{Action omission penalty:} detects actions that appear plausible locally but skip necessary causal steps.
\end{itemize}

At the episode level, the judge adds compact global signals for efficiency, consistency, and completeness~\citep{han2026swetrace}. These signals complement local turn rewards by discouraging trajectories that eventually succeed through inefficient, incoherent, or incomplete behavior:
\begin{itemize}
    \item \textbf{Efficiency:} penalizes redundant or repetitive execution.
    \item \textbf{Consistency:} checks whether the agent remains aligned with the original task.
    \item \textbf{Completeness:} measures whether required steps have been covered.
\end{itemize}

Given an embodied trajectory $\tau$ with $T$ evaluated action turns, the final reward is composed as:
\begin{equation}
R(\tau)=
\sum_{t=1}^{T}\hat{r}_{t}
+ \lambda_{\mathrm{eff}} R_{\mathrm{eff}}(\tau)
+ \lambda_{\mathrm{cons}} R_{\mathrm{cons}}(\tau)
+ \lambda_{\mathrm{comp}} R_{\mathrm{comp}}(\tau),
\label{eq:multi_tier_reward}
\end{equation}
where $\hat{r}_{t}$ is the effective turn-level reward after skill-aware routing, rule-based checks, LLM judgment, and omission penalties. $R_{\mathrm{eff}}$, $R_{\mathrm{cons}}$, and $R_{\mathrm{comp}}$ denote episode-level efficiency, consistency, and completeness rewards computed over the full trajectory. This formulation turns LLM-as-Judge from a static evaluator into a structured reward generator for embodied agent optimization~\citep{zheng2023judging}.

\subsubsection{Meta-Judge for Reasoning-Level Reward Audit}
\label{subsec:meta_judge_audit}

The second component in Figure~\ref{fig:judge_overview_v9} audits the reliability of the reward signal. In practice, LLM-as-Judge outputs can contain scoring mistakes, missed evidence, rubric misapplication, or plausible but unsupported rationales~\citep{silva2026metajudging}. This risk is amplified in embodied settings, where the judge must reason over physical preconditions, tool constraints, temporal order, and task-specific preferences.

To address this issue, Meta-Judge does not directly judge whether the embodied agent acted correctly. Instead, it receives the first-order judge output, the highlighted turn, and the full trajectory context as audit evidence, and then asks whether the judge's score and reasoning are reliable under the relevant scoring rubric. For each audited turn, Meta-Judge scores judgment quality along five dimensions:
\begin{itemize}
    \item \textbf{Accuracy:} whether the assigned reward score is consistent with the skill-specific scoring rubric and supported by the audited trajectory evidence.
    \item \textbf{Logical soundness:} whether the reasoning forms a valid chain from trajectory evidence, through rubric application, to the final reward decision, without unsupported jumps or contradictions.
    \item \textbf{Completeness:} whether the judge covers the key embodied checks required for the audited turn, including tool choice, arguments, temporal preconditions, physical constraints, capability boundaries, and omitted or redundant actions.
    \item \textbf{Clarity:} whether the explanation states the evidence, applied rule, and score rationale in a structured and unambiguous way.
    \item \textbf{Feedback value:} whether the reasoning exposes sufficiently localized evidence and rule usage for downstream Meta-Judge filtering and prompt refinement, rather than providing only a generic score justification.
\end{itemize}

This second-order audit is necessary because outcome accuracy and rationale quality may diverge: a judge can produce a seemingly correct score for the wrong reason~\citep{wang2026outcome}. These dimensions are aggregated into an overall quality score:
\begin{equation}
Q(x_t)=\sum_{k=1}^{5} w_k q_k,
\label{eq:meta_quality}
\end{equation}
where $x_t$ denotes the audited judge output, $q_k$ is the score of the $k$-th audit dimension, and $w_k$ is its weight. A sample is marked as a low-quality judge case when:
\begin{equation}
\mathrm{LowQualityJudgeCase}(x_t)=\mathbb{I}[Q(x_t)<\theta].
\label{eq:low_quality_case}
\end{equation}

These low-quality judge cases preserve diagnostic feedback rather than only binary error labels. They identify where the reward prompt is underspecified, ambiguous, or misaligned with embodied execution constraints, and provide the optimization signal for the next stage~\citep{li2025multiagent}.

\subsubsection{Multi-Agent Self-Evolution from Judge Audit Signals}
\label{subsec:structured_reward_optimization}

The third component in Figure~\ref{fig:judge_overview_v9} converts low-quality judge cases into localized prompt updates. The goal is to improve the reward engine itself rather than treating judge errors as fixed noise. Generic prompt optimization methods usually optimize a monolithic prompt with task-level feedback~\citep{yang2024opro,khattab2023dspy}. In our setting, however, the reward prompt contains skill-specific rubrics, temporal precondition rules, reasoning examples, and output constraints. A global rewrite can repair one failure while damaging another stable skill. We therefore treat the reward prompt as editable structured components, following the broader idea of modular textual parameters and localized textual modification from execution feedback~\citep{he2026learning}.

The optimization loop is implemented as a multi-agent workflow. Each module handles one stage of the update process:
\begin{itemize}
    \item \textbf{Cluster:} groups low-quality judge cases by skill and failure type.
    \item \textbf{Analyzer:} identifies the defective rubric component and produces a structured revision plan.
    \item \textbf{Refiner:} applies localized edits to the relevant rubric or examples.
    \item \textbf{Validator:} re-evaluates the revised prompt on the full validation set and accepts the update only when it improves overall quality.
\end{itemize}

If a candidate update hurts full-set performance, per-skill behavior, or Meta-Judge quality, the system rolls back to the previous prompt snapshot. This makes prompt self-evolution auditable and controlled: the structured revision plan records what should be changed and why, while validation prevents overfitting to isolated bad cases.

Under the current validation setting, the initial Judge Model achieves roughly 60\% human alignment, while the Meta-Judge-driven self-evolution process improves alignment to above 90\%. This gain reflects the coupled effect of the full loop: LLM-as-Judge produces decomposed rewards, Meta-Judge turns unreliable judgments into diagnostic cases, and the multi-agent optimizer converts these cases into validated prompt updates.

Overall, the proposed reward engine closes the loop around reward production. It not only generates dense multi-tier rewards for embodied trajectories, but also audits and improves the judging process that produces those rewards. This allows the evaluation system to remain reliable as embodied skills, task distributions, and agent behaviors evolve.

